Low-shot Visual Recognition by Shrinking and Hallucinating Features

Low-shot visual learning---the ability to recognize novel object categories from very few examples---is a hallmark of human visual intelligence. Existing machine learning approaches fail to generalize in the same way. To make progress on this foundational problem, we present a low-shot learning benchmark on complex images that mimics challenges faced by recognition systems in the wild. We then propose a) representation regularization techniques, and b) techniques to hallucinate additional training examples for data-starved classes. Together, our methods improve the effectiveness of convolutional networks in low-shot learning, improving the one-shot accuracy on novel classes by 2.3x on the challenging ImageNet dataset.

==> acknowledgements.tex <==
\subsection*{Acknowledgements}
We thank Piotr Dollar and Larry Zitnick for the many insightful discussions.


==> doman.tex <==
\begin{tabular}{lccccccccc}
\toprule
$n$ & Baseline & Batch SGM & $L_2$ & Triplet & SGM & Dropout & L1 & Multiverse & DeCov\\
\midrule
\multicolumn{10}{c}{Novel classes}\\
\midrule
1 & 14.85 $\pm$ 0.90 & 28.19 $\pm$ 1.93 & 27.48 $\pm$ 1.76 & 12.90 $\pm$ 0.96 & 28.70 $\pm$ 2.24 & 18.25 $\pm$ 1.12 & 25.26 $\pm$ 2.12 & 15.20 $\pm$ 0.49 & 15.46 $\pm$ 1.35\\
2 & 32.79 $\pm$ 1.64 & 45.89 $\pm$ 1.49 & 45.38 $\pm$ 2.59 & 29.62 $\pm$ 1.53 & 45.96 $\pm$ 2.18 & 36.13 $\pm$ 1.65 & 41.72 $\pm$ 0.95 & 32.14 $\pm$ 1.02 & 35.54 $\pm$ 1.18\\
5 & 53.77 $\pm$ 1.24 & 63.17 $\pm$ 1.39 & 62.53 $\pm$ 1.34 & 52.29 $\pm$ 1.21 & 63.59 $\pm$ 1.81 & 57.47 $\pm$ 1.42 & 58.82 $\pm$ 1.14 & 54.78 $\pm$ 1.08 & 59.12 $\pm$ 1.33\\
10 & 62.78 $\pm$ 0.48 & 70.23 $\pm$ 0.81 & 69.56 $\pm$ 0.46 & 63.59 $\pm$ 0.84 & 70.44 $\pm$ 0.89 & 67.35 $\pm$ 0.96 & 65.56 $\pm$ 0.65 & 65.96 $\pm$ 0.42 & 69.12 $\pm$ 0.55\\
20 & 68.00 $\pm$ 0.64 & 74.31 $\pm$ 0.34 & 73.90 $\pm$ 0.46 & 69.92 $\pm$ 0.63 & 74.17 $\pm$ 0.09 & 74.19 $\pm$ 0.56 & 69.69 $\pm$ 1.11 & 73.46 $\pm$ 0.68 & 74.17 $\pm$ 0.62\\
\midrule
\multicolumn{10}{c}{Base classes}\\
\midrule
1 & 91.67 $\pm$ 0.28 & 94.07 $\pm$ 0.11 & 93.97 $\pm$ 0.29 & 95.31 $\pm$ 0.27 & 94.18 $\pm$ 0.43 & 95.37 $\pm$ 0.07 & 89.58 $\pm$ 0.63 & 96.18 $\pm$ 0.15 & 95.92 $\pm$ 0.40\\
2 & 86.89 $\pm$ 0.35 & 91.01 $\pm$ 0.33 & 90.96 $\pm$ 0.43 & 93.37 $\pm$ 0.17 & 91.17 $\pm$ 0.61 & 93.57 $\pm$ 0.17 & 85.22 $\pm$ 0.39 & 95.13 $\pm$ 0.18 & 94.34 $\pm$ 0.39\\
5 & 81.49 $\pm$ 0.71 & 88.31 $\pm$ 0.58 & 88.10 $\pm$ 0.44 & 88.36 $\pm$ 0.28 & 88.48 $\pm$ 0.53 & 89.91 $\pm$ 0.35 & 82.41 $\pm$ 0.53 & 92.60 $\pm$ 0.41 & 90.40 $\pm$ 0.44\\
10 & 80.32 $\pm$ 0.76 & 87.39 $\pm$ 0.19 & 87.21 $\pm$ 0.51 & 85.76 $\pm$ 0.24 & 87.64 $\pm$ 0.30 & 87.40 $\pm$ 0.54 & 82.32 $\pm$ 0.62 & 90.03 $\pm$ 0.26 & 88.44 $\pm$ 0.45\\
20 & 80.11 $\pm$ 0.88 & 87.40 $\pm$ 0.35 & 87.07 $\pm$ 0.44 & 84.86 $\pm$ 0.40 & 87.40 $\pm$ 0.16 & 85.56 $\pm$ 0.45 & 82.44 $\pm$ 0.50 & 87.97 $\pm$ 0.42 & 87.56 $\pm$ 0.27\\
\bottomrule
\end{tabular}


==> doman_base_top5.tex <==
\begin{tabular}{lccccccccc}
\toprule
n & Baseline & Batch SGM & $L_2$ & Triplet & SGM & Dropout & L1 & Multiverse & DeCov\\
\midrule
1 & 91.67 $\pm$ 0.28 & 94.07 $\pm$ 0.11 & 93.97 $\pm$ 0.29 & 95.31 $\pm$ 0.27 & 94.18 $\pm$ 0.43 & 95.37 $\pm$ 0.07 & 89.58 $\pm$ 0.63 & 96.18 $\pm$ 0.15 & 95.92 $\pm$ 0.40\\
2 & 86.89 $\pm$ 0.35 & 91.01 $\pm$ 0.33 & 90.96 $\pm$ 0.43 & 93.37 $\pm$ 0.17 & 91.17 $\pm$ 0.61 & 93.57 $\pm$ 0.17 & 85.22 $\pm$ 0.39 & 95.13 $\pm$ 0.18 & 94.34 $\pm$ 0.39\\
5 & 81.49 $\pm$ 0.71 & 88.31 $\pm$ 0.58 & 88.10 $\pm$ 0.44 & 88.36 $\pm$ 0.28 & 88.48 $\pm$ 0.53 & 89.91 $\pm$ 0.35 & 82.41 $\pm$ 0.53 & 92.60 $\pm$ 0.41 & 90.40 $\pm$ 0.44\\
10 & 80.32 $\pm$ 0.76 & 87.39 $\pm$ 0.19 & 87.21 $\pm$ 0.51 & 85.76 $\pm$ 0.24 & 87.64 $\pm$ 0.30 & 87.40 $\pm$ 0.54 & 82.32 $\pm$ 0.62 & 90.03 $\pm$ 0.26 & 88.44 $\pm$ 0.45\\
20 & 80.11 $\pm$ 0.88 & 87.40 $\pm$ 0.35 & 87.07 $\pm$ 0.44 & 84.86 $\pm$ 0.40 & 87.40 $\pm$ 0.16 & 85.56 $\pm$ 0.45 & 82.44 $\pm$ 0.50 & 87.97 $\pm$ 0.42 & 87.56 $\pm$ 0.27\\
\bottomrule
\end{tabular}


==> doman_novel_top5.tex <==
\begin{tabular}{lccccccccc}
\toprule
n & Baseline & Batch SGM & $L_2$ & Triplet & SGM & Dropout & L1 & Multiverse & DeCov\\
\midrule
1 & 14.85 $\pm$ 0.90 & 28.19 $\pm$ 1.93 & 27.48 $\pm$ 1.76 & 12.90 $\pm$ 0.96 & 28.70 $\pm$ 2.24 & 18.25 $\pm$ 1.12 & 25.26 $\pm$ 2.12 & 15.20 $\pm$ 0.49 & 15.46 $\pm$ 1.35\\
2 & 32.79 $\pm$ 1.64 & 45.89 $\pm$ 1.49 & 45.38 $\pm$ 2.59 & 29.62 $\pm$ 1.53 & 45.96 $\pm$ 2.18 & 36.13 $\pm$ 1.65 & 41.72 $\pm$ 0.95 & 32.14 $\pm$ 1.02 & 35.54 $\pm$ 1.18\\
5 & 53.77 $\pm$ 1.24 & 63.17 $\pm$ 1.39 & 62.53 $\pm$ 1.34 & 52.29 $\pm$ 1.21 & 63.59 $\pm$ 1.81 & 57.47 $\pm$ 1.42 & 58.82 $\pm$ 1.14 & 54.78 $\pm$ 1.08 & 59.12 $\pm$ 1.33\\
10 & 62.78 $\pm$ 0.48 & 70.23 $\pm$ 0.81 & 69.56 $\pm$ 0.46 & 63.59 $\pm$ 0.84 & 70.44 $\pm$ 0.89 & 67.35 $\pm$ 0.96 & 65.56 $\pm$ 0.65 & 65.96 $\pm$ 0.42 & 69.12 $\pm$ 0.55\\
20 & 68.00 $\pm$ 0.64 & 74.31 $\pm$ 0.34 & 73.90 $\pm$ 0.46 & 69.92 $\pm$ 0.63 & 74.17 $\pm$ 0.09 & 74.19 $\pm$ 0.56 & 69.69 $\pm$ 1.11 & 73.46 $\pm$ 0.68 & 74.17 $\pm$ 0.62\\
\bottomrule
\end{tabular}


==> plots/top1_all.tex <==
\begin{tabular}{llccccc}
\toprule
Representation & Lowshot phase & n=1 & 2 & 5 & 10 & 20 \\
\midrule
Baseline & Classifier & 29.16 & 33.53 & 41.57 & 46.33 & 49.74 \\
Baseline & Generation$^*$ + Classifier & 33.60 & 36.83 & 42.11 & 46.70 & 51.65 \\
SGM$^*$ & Classifier & 31.83 & 36.73 & 44.45 & 48.79 & 51.77 \\
SGM$^*$ & Generation$^*$ + Classifier & 34.12 & 38.09 & 44.50 & 48.82 & 51.79 \\
Batch SGM$^*$ & Classifier & 31.84 & 36.78 & 44.63 & 49.05 & 52.11 \\
Triplets & Classifier & 28.09 & 32.16 & 37.17 & 39.85 & 41.47 \\
L2$^*$ & Classifier & 33.18 & 38.21 & 44.07 & 46.74 & 48.37 \\
Dropout & Classifier & 31.29 & 36.05 & 42.12 & 45.33 & 47.53 \\
Decov & Classifier & 30.13 & 34.21 & 43.61 & 48.65 & 51.70 \\
L1$^*$ & Classifier & 30.37 & 35.40 & 42.82 & 46.80 & 49.39 \\
Multiverse & Classifier & 30.19 & 33.11 & 40.80 & 46.67 & 50.92 \\
Baseline & Model Regression & 29.70 & 33.84 & 38.15 & 39.23 & 40.21 \\
Baseline & Matching Network & 30.08 & 34.78 & 41.74 & 45.81 & 48.81 \\
Baseline-ft & Classifier & 28.14 & 31.55 & 39.61 & 45.04 & 48.63 \\
Baseline (Resnet 50) & Classifier & 36.33 & 42.95 & 52.71 & 57.79 & 61.01 \\
Baseline (Resnet 50) & Generation$^*$ + Classifier & 40.86 & 45.65 & 51.90 & 56.74 & 61.03 \\
SGM (Resnet 50) & Classifier & 38.73 & 45.06 & 53.40 & 57.90 & 60.93 \\
SGM (Resnet 50) & Generation$^*$ + Classifier & 41.05 & 45.76 & 53.39 & 57.90 & 60.92 \\
\bottomrule
\end{tabular}


==> plots/top1_all_std.tex <==
\begin{tabular}{llccccc}
\toprule
Representation & Lowshot phase & n=1 & 2 & 5 & 10 & 20 \\
\midrule
Baseline & Classifier & 0.10 & 0.19 & 0.26 & 0.39 & 0.12 \\
Baseline & Generation$^*$ + Classifier & 0.12 & 0.20 & 0.29 & 0.29 & 0.17 \\
SGM$^*$ & Classifier & 0.17 & 0.17 & 0.30 & 0.26 & 0.28 \\
SGM$^*$ & Generation$^*$ + Classifier & 0.28 & 0.22 & 0.24 & 0.29 & 0.33 \\
Batch SGM$^*$ & Classifier & 0.25 & 0.30 & 0.31 & 0.23 & 0.24 \\
Triplets & Classifier & 0.08 & 0.28 & 0.30 & 0.17 & 0.22 \\
L2$^*$ & Classifier & 0.16 & 0.40 & 0.28 & 0.20 & 0.20 \\
Dropout & Classifier & 0.13 & 0.37 & 0.49 & 0.30 & 0.18 \\
Decov & Classifier & 0.08 & 0.17 & 0.20 & 0.27 & 0.26 \\
L1$^*$ & Classifier & 0.11 & 0.31 & 0.24 & 0.33 & 0.13 \\
Multiverse & Classifier & 0.09 & 0.13 & 0.36 & 0.36 & 0.15 \\
Baseline & Model Regression & 0.10 & 0.25 & 0.32 & 0.21 & 0.20 \\
Baseline & Generation$^*$ + Classifier & 0.43 & 0.47 & 0.36 & 0.30 & 0.27 \\
Baseline-ft & Classifier & 0.11 & 0.17 & 0.43 & 0.19 & 0.25 \\
Baseline (Resnet 50) & Classifier & 0.07 & 0.38 & 0.28 & 0.26 & 0.18 \\
Baseline (Resnet 50) & Generation$^*$ + Classifier & 0.14 & 0.25 & 0.42 & 0.26 & 0.25 \\
SGM (Resnet 50) & Classifier & 0.11 & 0.36 & 0.29 & 0.21 & 0.26 \\
SGM (Resnet 50) & Generation$^*$ + Classifier & 0.21 & 0.30 & 0.24 & 0.24 & 0.24 \\
\bottomrule
\end{tabular}


==> plots/top1_novel.tex <==
\begin{tabular}{llccccc}
\toprule
Representation & Lowshot phase & n=1 & 2 & 5 & 10 & 20 \\
\midrule
Baseline & Classifier & 2.77 & 10.78 & 26.38 & 35.46 & 41.49 \\
Baseline & Generation$^*$ + Classifier & 9.17 & 15.85 & 25.47 & 33.21 & 40.41 \\
SGM$^*$ & Classifier & 4.14 & 13.08 & 27.83 & 36.04 & 41.36 \\
SGM$^*$ & Generation$^*$ + Classifier & 9.85 & 17.32 & 27.89 & 36.17 & 41.42 \\
Batch SGM$^*$ & Classifier & 4.16 & 13.01 & 28.12 & 36.56 & 42.07 \\
Triplets & Classifier & 6.22 & 15.13 & 24.58 & 28.73 & 31.14 \\
L2$^*$ & Classifier & 7.14 & 16.75 & 27.73 & 32.32 & 35.11 \\
Dropout & Classifier & 7.22 & 16.58 & 27.77 & 33.28 & 36.80 \\
Decov & Classifier & 1.75 & 8.83 & 26.52 & 36.33 & 41.87 \\
L1$^*$ & Classifier & 4.88 & 14.40 & 28.54 & 35.59 & 39.90 \\
Multiverse & Classifier & 1.55 & 6.47 & 19.93 & 31.04 & 39.65 \\
Baseline & Model Regression & 5.73 & 15.62 & 30.53 & 38.25 & 43.57 \\
Baseline & Matching Network & 18.33 & 23.87 & 31.08 & 35.27 & 38.45 \\
Baseline-ft & Classifier & 2.26 & 8.52 & 23.97 & 34.42 & 40.96 \\
Baseline (Resnet 50) & Classifier & 6.82 & 18.37 & 36.55 & 46.15 & 51.99 \\
Baseline (Resnet 50) & Generation$^*$ + Classifier & 16.58 & 25.38 & 36.16 & 44.53 & 52.06 \\
SGM (Resnet 50) & Classifier & 10.23 & 21.45 & 37.25 & 46.00 & 51.83 \\
SGM (Resnet 50) & Generation$^*$ + Classifier & 15.77 & 24.43 & 37.22 & 45.96 & 51.82 \\
\bottomrule
\end{tabular}


==> plots/top1_novel_std.tex <==
\begin{tabular}{llccccc}
\toprule
Representation & Lowshot phase & n=1 & 2 & 5 & 10 & 20 \\
\midrule
Baseline & Classifier & 0.22 & 0.23 & 0.55 & 0.61 & 0.19 \\
Baseline & Generation$^*$ + Classifier & 0.21 & 0.31 & 0.51 & 0.43 & 0.27 \\
SGM$^*$ & Classifier & 0.28 & 0.14 & 0.53 & 0.40 & 0.41 \\
SGM$^*$ & Generation$^*$ + Classifier & 0.43 & 0.36 & 0.42 & 0.41 & 0.47 \\
Batch SGM$^*$ & Classifier & 0.33 & 0.40 & 0.49 & 0.35 & 0.47 \\
Triplets & Classifier & 0.13 & 0.37 & 0.54 & 0.32 & 0.38 \\
L2$^*$ & Classifier & 0.28 & 0.60 & 0.48 & 0.34 & 0.30 \\
Dropout & Classifier & 0.24 & 0.61 & 0.84 & 0.52 & 0.42 \\
Decov & Classifier & 0.09 & 0.24 & 0.30 & 0.38 & 0.37 \\
L1$^*$ & Classifier & 0.23 & 0.46 & 0.51 & 0.59 & 0.25 \\
Multiverse & Classifier & 0.17 & 0.19 & 0.56 & 0.59 & 0.29 \\
Baseline & Model Regression & 0.15 & 0.41 & 0.52 & 0.38 & 0.39 \\
Baseline & Generation$^*$ + Classifier & 0.52 & 0.87 & 0.31 & 0.30 & 0.30 \\
Baseline-ft & Classifier & 0.23 & 0.29 & 0.68 & 0.35 & 0.43 \\
Baseline (Resnet 50) & Classifier & 0.07 & 0.62 & 0.49 & 0.35 & 0.23 \\
Baseline (Resnet 50) & Generation$^*$ + Classifier & 0.26 & 0.42 & 0.73 & 0.43 & 0.36 \\
SGM (Resnet 50) & Classifier & 0.18 & 0.56 & 0.43 & 0.33 & 0.44 \\
SGM (Resnet 50) & Generation$^*$ + Classifier & 0.28 & 0.42 & 0.38 & 0.39 & 0.43 \\
\bottomrule
\end{tabular}


==> plots/top5_all2.tex <==
\begin{tabular}{llccccc}
\toprule
Representation & Lowshot phase & n=1 & 2 & 5 & 10 & 20 \\
\midrule
Baseline & Classifier & 43.02 & 54.29 & 67.17 & 72.75 & 75.86 \\
Baseline & Generation + Classifier & 52.35 & 59.42 & 67.53 & 72.65 & 76.91 \\
SGM & Classifier & 49.37 & 60.52 & 71.34 & 75.75 & 78.10 \\
SGM & Generation + Classifier & 54.31 & 62.12 & 71.33 & 75.81 & 78.12 \\
Batch SGM & Classifier & 49.32 & 60.52 & 71.44 & 75.89 & 78.48 \\
Triplets & Classifier & 47.64 & 57.09 & 65.18 & 68.44 & 70.20 \\
L2 & Classifier & 52.65 & 63.05 & 71.48 & 74.79 & 76.41 \\
Dropout & Classifier & 50.07 & 59.74 & 68.76 & 72.70 & 74.65 \\
Decov & Classifier & 43.29 & 55.74 & 70.08 & 75.35 & 77.90 \\
L1 & Classifier & 47.08 & 58.54 & 69.21 & 73.68 & 76.06 \\
Multiverse & Classifier & 44.06 & 54.22 & 66.98 & 73.16 & 76.93 \\
Baseline & Model Regression & 46.41 & 56.72 & 66.75 & 70.35 & 72.00 \\
Baseline & Matching Network & 54.97 & 61.52 & 69.27 & 73.38 & 76.22 \\
Baseline-ft & Classifier & 41.73 & 51.68 & 64.95 & 71.23 & 74.51 \\
Baseline (Resnet 50) & Classifier & 54.05 & 67.65 & 79.07 & 83.15 & 85.37 \\
Baseline (Resnet 50) & Generation + Classifier & 63.14 & 71.45 & 78.76 & 82.55 & 85.35 \\
SGM (Resnet 50) & Classifier & 60.02 & 71.28 & 79.95 & 83.27 & 85.19 \\
SGM (Resnet 50) & Generation + Classifier & 63.60 & 71.53 & 79.95 & 83.27 & 85.16 \\
\bottomrule
\end{tabular}


==> plots/top5_all_std.tex <==
\begin{tabular}{llccccc}
\toprule
Representation & Lowshot phase & n=1 & 2 & 5 & 10 & 20 \\
\midrule
Baseline & Classifier & 0.10 & 0.28 & 0.27 & 0.23 & 0.06 \\
Baseline & Generation$^*$ + Classifier & 0.33 & 0.36 & 0.23 & 0.27 & 0.08 \\
SGM$^*$ & Classifier & 0.28 & 0.29 & 0.18 & 0.28 & 0.26 \\
SGM$^*$ & Generation$^*$ + Classifier & 0.24 & 0.33 & 0.20 & 0.23 & 0.27 \\
Batch SGM$^*$ & Classifier & 0.35 & 0.32 & 0.22 & 0.25 & 0.26 \\
Triplets & Classifier & 0.36 & 0.40 & 0.22 & 0.37 & 0.21 \\
L2$^*$ & Classifier & 0.41 & 0.37 & 0.26 & 0.26 & 0.18 \\
Dropout & Classifier & 0.45 & 0.34 & 0.20 & 0.28 & 0.17 \\
Decov & Classifier & 0.29 & 0.16 & 0.20 & 0.42 & 0.24 \\
L1$^*$ & Classifier & 0.11 & 0.32 & 0.19 & 0.35 & 0.20 \\
Multiverse & Classifier & 0.24 & 0.27 & 0.15 & 0.34 & 0.28 \\
Baseline & Model Regression & 0.19 & 0.30 & 0.25 & 0.29 & 0.14 \\
Baseline & Generation$^*$ + Classifier & 0.37 & 0.35 & 0.23 & 0.35 & 0.20 \\
Baseline-ft & Classifier & 0.34 & 0.43 & 0.14 & 0.23 & 0.21 \\
Baseline (Resnet 50) & Classifier & 0.30 & 0.50 & 0.12 & 0.25 & 0.13 \\
Baseline (Resnet 50) & Generation$^*$ + Classifier & 0.44 & 0.30 & 0.12 & 0.16 & 0.16 \\
SGM (Resnet 50) & Classifier & 0.19 & 0.32 & 0.10 & 0.18 & 0.16 \\
SGM (Resnet 50) & Generation$^*$ + Classifier & 0.33 & 0.17 & 0.11 & 0.17 & 0.18 \\
\bottomrule
\end{tabular}


==> plots/top5_novel2.tex <==
\begin{tabular}{llccccc}
\toprule
Representation & Lowshot phase & n=1 & 2 & 5 & 10 & 20 \\
\midrule
Baseline & Classifier & 14.10 & 33.34 & 56.20 & 66.15 & 71.52 \\
Baseline & Generation + Classifier & 29.68 & 42.15 & 56.13 & 64.52 & 70.56 \\
SGM & Classifier & 23.14 & 42.37 & 61.68 & 69.60 & 73.76 \\
SGM & Generation + Classifier & 32.80 & 46.37 & 61.70 & 69.71 & 73.81 \\
Batch SGM & Classifier & 22.97 & 42.35 & 61.91 & 69.91 & 74.45 \\
Triplets & Classifier & 24.54 & 41.82 & 56.04 & 61.34 & 64.17 \\
L2 & Classifier & 29.08 & 47.42 & 62.33 & 67.96 & 70.63 \\
Dropout & Classifier & 26.83 & 43.92 & 59.62 & 66.21 & 69.46 \\
Decov & Classifier & 12.95 & 33.94 & 59.25 & 68.87 & 73.41 \\
L1 & Classifier & 20.77 & 40.80 & 59.80 & 67.52 & 71.55 \\
Multiverse & Classifier & 13.65 & 30.61 & 52.54 & 63.80 & 71.06 \\
Baseline & Model Regression & 20.71 & 39.39 & 59.63 & 68.54 & 73.54 \\
Baseline & Matching Network & 41.27 & 51.25 & 62.13 & 67.82 & 71.78 \\
Baseline-ft & Classifier & 12.48 & 29.49 & 53.08 & 64.58 & 70.41 \\
Baseline (Resnet 50) & Classifier & 28.16 & 51.03 & 71.01 & 78.39 & 82.32 \\
Baseline (Resnet 50) & Generation + Classifier & 44.76 & 58.98 & 71.37 & 77.65 & 82.30 \\
SGM (Resnet 50) & Classifier & 37.81 & 57.08 & 72.78 & 79.09 & 82.61 \\
SGM (Resnet 50) & Generation + Classifier & 45.11 & 58.83 & 72.76 & 79.09 & 82.61 \\
\bottomrule
\end{tabular}


==> plots/top5_novel_std.tex <==
\begin{tabular}{llccccc}
\toprule
Representation & Lowshot phase & n=1 & 2 & 5 & 10 & 20 \\
\midrule
Baseline & Classifier & 0.20 & 0.42 & 0.52 & 0.40 & 0.21 \\
Baseline & Generation$^*$ + Classifier & 0.58 & 0.52 & 0.32 & 0.44 & 0.17 \\
SGM$^*$ & Classifier & 0.43 & 0.51 & 0.32 & 0.51 & 0.40 \\
SGM$^*$ & Generation$^*$ + Classifier & 0.40 & 0.55 & 0.34 & 0.37 & 0.34 \\
Batch SGM$^*$ & Classifier & 0.62 & 0.51 & 0.35 & 0.38 & 0.39 \\
Triplets & Classifier & 0.58 & 0.68 & 0.30 & 0.60 & 0.34 \\
L2$^*$ & Classifier & 0.62 & 0.57 & 0.42 & 0.42 & 0.28 \\
Dropout & Classifier & 0.72 & 0.47 & 0.31 & 0.44 & 0.32 \\
Decov & Classifier & 0.51 & 0.21 & 0.30 & 0.68 & 0.38 \\
L1$^*$ & Classifier & 0.18 & 0.48 & 0.26 & 0.58 & 0.34 \\
Multiverse & Classifier & 0.42 & 0.43 & 0.29 & 0.55 & 0.36 \\
Baseline & Model Regression & 0.29 & 0.43 & 0.38 & 0.49 & 0.17 \\
Baseline & Generation$^*$ + Classifier & 0.45 & 0.45 & 0.25 & 0.54 & 0.26 \\
Baseline-ft & Classifier & 0.53 & 0.63 & 0.17 & 0.40 & 0.28 \\
Baseline (Resnet 50) & Classifier & 0.49 & 0.77 & 0.24 & 0.41 & 0.20 \\
Baseline (Resnet 50) & Generation$^*$ + Classifier & 0.67 & 0.47 & 0.19 & 0.25 & 0.25 \\
SGM (Resnet 50) & Classifier & 0.30 & 0.54 & 0.16 & 0.27 & 0.28 \\
SGM (Resnet 50) & Generation$^*$ + Classifier & 0.54 & 0.25 & 0.20 & 0.25 & 0.30 \\
\bottomrule
\end{tabular}


==> root.tex <==
\begin{tabular}{lccccccccc}
\toprule
$n$ & Baseline & Batch SGM & $L_2$ & Triplet & SGM & Dropout & L1  & Multiverse & DeCov\\
\midrule
\multicolumn{10}{c}{Novel classes}\\
\midrule
1 & 4.32 $\pm$ 0.32 & 18.78 $\pm$ 0.52 & 17.86 $\pm$ 0.69 & 8.52 $\pm$ 0.37 & 18.80 $\pm$ 0.59 & 12.17 $\pm$ 0.33 & 8.43 $\pm$ 0.27 & 8.67 $\pm$ 0.30 & 9.07 $\pm$ 0.32\\
2 & 15.31 $\pm$ 0.44 & 33.85 $\pm$ 0.68 & 33.32 $\pm$ 0.78 & 22.79 $\pm$ 0.64 & 34.07 $\pm$ 0.65 & 26.48 $\pm$ 0.59 & 22.28 $\pm$ 0.35 & 22.44 $\pm$ 0.63 & 26.45 $\pm$ 0.27\\
5 & 37.61 $\pm$ 0.39 & 48.61 $\pm$ 0.33 & 49.57 $\pm$ 0.23 & 43.39 $\pm$ 0.16 & 48.94 $\pm$ 0.30 & 46.12 $\pm$ 0.41 & 44.11 $\pm$ 0.45 & 43.08 $\pm$ 0.41 & 48.24 $\pm$ 0.54\\
10 & 51.45 $\pm$ 0.25 & 54.98 $\pm$ 0.20 & 56.55 $\pm$ 0.15 & 52.85 $\pm$ 0.31 & 55.46 $\pm$ 0.35 & 56.19 $\pm$ 0.32 & 56.13 $\pm$ 0.23 & 54.54 $\pm$ 0.51 & 56.78 $\pm$ 0.41\\
20 & 61.07 $\pm$ 0.19 & 58.29 $\pm$ 0.21 & 60.08 $\pm$ 0.34 & 58.35 $\pm$ 0.26 & 58.94 $\pm$ 0.24 & 62.04 $\pm$ 0.34 & 63.36 $\pm$ 0.20 & 62.12 $\pm$ 0.44 & 61.42 $\pm$ 0.26\\
\midrule
\multicolumn{10}{c}{Base classes}\\
\midrule
1 & 87.81 $\pm$ 0.07 & 86.32 $\pm$ 0.15 & 86.96 $\pm$ 0.04 & 84.39 $\pm$ 0.04 & 86.61 $\pm$ 0.10 & 86.53 $\pm$ 0.04 & 87.75 $\pm$ 0.08 & 88.33 $\pm$ 0.09 & 87.53 $\pm$ 0.10\\
2 & 87.21 $\pm$ 0.10 & 84.16 $\pm$ 0.21 & 84.58 $\pm$ 0.13 & 82.42 $\pm$ 0.11 & 84.37 $\pm$ 0.12 & 84.68 $\pm$ 0.16 & 86.57 $\pm$ 0.05 & 87.30 $\pm$ 0.08 & 85.62 $\pm$ 0.09\\
5 & 84.89 $\pm$ 0.12 & 82.31 $\pm$ 0.11 & 82.21 $\pm$ 0.21 & 77.97 $\pm$ 0.14 & 82.47 $\pm$ 0.09 & 81.00 $\pm$ 0.14 & 83.35 $\pm$ 0.09 & 84.54 $\pm$ 0.18 & 81.83 $\pm$ 0.11\\
10 & 82.33 $\pm$ 0.03 & 82.02 $\pm$ 0.10 & 81.80 $\pm$ 0.17 & 76.20 $\pm$ 0.12 & 82.13 $\pm$ 0.11 & 79.20 $\pm$ 0.12 & 81.05 $\pm$ 0.10 & 82.01 $\pm$ 0.14 & 80.78 $\pm$ 0.12\\
20 & 80.56 $\pm$ 0.14 & 81.96 $\pm$ 0.15 & 81.74 $\pm$ 0.19 & 75.59 $\pm$ 0.11 & 82.10 $\pm$ 0.11 & 78.48 $\pm$ 0.18 & 79.94 $\pm$ 0.17 & 80.43 $\pm$ 0.15 & 80.61 $\pm$ 0.16\\
\bottomrule
\end{tabular}


==> root_base_top5.tex <==
\begin{tabular}{lccccccccc}
\toprule
n & Baseline & Batched SGM & $L_2$ & Triplet & SGM & Dropout & L1  & Multiverse & DeCov\\
\midrule
1 & 87.81 $\pm$ 0.07 & 86.32 $\pm$ 0.15 & 86.96 $\pm$ 0.04 & 84.39 $\pm$ 0.04 & 86.61 $\pm$ 0.10 & 86.53 $\pm$ 0.04 & 87.75 $\pm$ 0.08 & 88.33 $\pm$ 0.09 & 87.53 $\pm$ 0.10\\
2 & 87.21 $\pm$ 0.10 & 84.16 $\pm$ 0.21 & 84.58 $\pm$ 0.13 & 82.42 $\pm$ 0.11 & 84.37 $\pm$ 0.12 & 84.68 $\pm$ 0.16 & 86.57 $\pm$ 0.05 & 87.30 $\pm$ 0.08 & 85.62 $\pm$ 0.09\\
5 & 84.89 $\pm$ 0.12 & 82.31 $\pm$ 0.11 & 82.21 $\pm$ 0.21 & 77.97 $\pm$ 0.14 & 82.47 $\pm$ 0.09 & 81.00 $\pm$ 0.14 & 83.35 $\pm$ 0.09 & 84.54 $\pm$ 0.18 & 81.83 $\pm$ 0.11\\
10 & 82.33 $\pm$ 0.03 & 82.02 $\pm$ 0.10 & 81.80 $\pm$ 0.17 & 76.20 $\pm$ 0.12 & 82.13 $\pm$ 0.11 & 79.20 $\pm$ 0.12 & 81.05 $\pm$ 0.10 & 82.01 $\pm$ 0.14 & 80.78 $\pm$ 0.12\\
20 & 80.56 $\pm$ 0.14 & 81.96 $\pm$ 0.15 & 81.74 $\pm$ 0.19 & 75.59 $\pm$ 0.11 & 82.10 $\pm$ 0.11 & 78.48 $\pm$ 0.18 & 79.94 $\pm$ 0.17 & 80.43 $\pm$ 0.15 & 80.61 $\pm$ 0.16\\
\bottomrule
\end{tabular}


==> root_novel_top5.tex <==
\begin{tabular}{lccccccccc}
\toprule
n & Baseline & Batched SGM & $L_2$ & Triplet & SGM & Dropout & L1  & Multiverse & DeCov\\
\midrule
1 & 4.32 $\pm$ 0.32 & 18.78 $\pm$ 0.52 & 17.86 $\pm$ 0.69 & 8.52 $\pm$ 0.37 & 18.80 $\pm$ 0.59 & 12.17 $\pm$ 0.33 & 8.43 $\pm$ 0.27 & 8.67 $\pm$ 0.30 & 9.07 $\pm$ 0.32\\
2 & 15.31 $\pm$ 0.44 & 33.85 $\pm$ 0.68 & 33.32 $\pm$ 0.78 & 22.79 $\pm$ 0.64 & 34.07 $\pm$ 0.65 & 26.48 $\pm$ 0.59 & 22.28 $\pm$ 0.35 & 22.44 $\pm$ 0.63 & 26.45 $\pm$ 0.27\\
5 & 37.61 $\pm$ 0.39 & 48.61 $\pm$ 0.33 & 49.57 $\pm$ 0.23 & 43.39 $\pm$ 0.16 & 48.94 $\pm$ 0.30 & 46.12 $\pm$ 0.41 & 44.11 $\pm$ 0.45 & 43.08 $\pm$ 0.41 & 48.24 $\pm$ 0.54\\
10 & 51.45 $\pm$ 0.25 & 54.98 $\pm$ 0.20 & 56.55 $\pm$ 0.15 & 52.85 $\pm$ 0.31 & 55.46 $\pm$ 0.35 & 56.19 $\pm$ 0.32 & 56.13 $\pm$ 0.23 & 54.54 $\pm$ 0.51 & 56.78 $\pm$ 0.41\\
20 & 61.07 $\pm$ 0.19 & 58.29 $\pm$ 0.21 & 60.08 $\pm$ 0.34 & 58.35 $\pm$ 0.26 & 58.94 $\pm$ 0.24 & 62.04 $\pm$ 0.34 & 63.36 $\pm$ 0.20 & 62.12 $\pm$ 0.44 & 61.42 $\pm$ 0.26\\
\bottomrule
\end{tabular}

